Self-Supervised Learning for Monocular Depth Estimation from Aerial Imagery

Supervised learning based methods for monocular depth estimation usually require large amounts of extensively annotated training data. In the case of aerial imagery, this ground truth is particularly difficult to acquire. Therefore, in this paper, we present a method for self-supervised learning for monocular depth estimation from aerial imagery that does not require annotated training data. For this, we only use an image sequence from a single moving camera and learn to simultaneously estimate depth and pose information. By sharing the weights between pose and depth estimation, we achieve a relatively small model, which favors real-time application. We evaluate our approach on three diverse datasets and compare the results to conventional methods that estimate depth maps based on multi-view geometry. We achieve an accuracy {\delta}1.25 of up to 93.5 %. In addition, we have paid particular attention to the generalization of a trained model to unknown data and the self-improving capabilities of our approach. We conclude that, even though the results of monocular depth estimation are inferior to those achieved by conventional methods, they are well suited to provide a good initialization for methods that rely on image matching or to provide estimates in regions where image matching fails, e.g. occluded or texture-less regions.

==> chapters/05_discussion.tex <==
\section{Discussion of the experimental results}
\label{sec:discussion}

% KAO: Sloppy spacing ensures non-overfull lines. Can be removed if this is not an issue.
\sloppy 

\todo[color=blue!20!white, inline]{Boitu}
\todo[inline]{Max}

%Especially fine structures like vegetation and sharp edges are incorrectly represented by our model. 

%As shown in table \ref{tab:results_of_combined_model}, our model provides useful results, although these vary depending on the dataset. Especially the urban dataset delivers significantly worse results. A possible explanation for this is that the poorer image quality affects the depth estimation. Another indication of this is the objectively lower quality of the ground truth produced by COLMAP. Corresponding artifacts are visible in figure \ref{fig:qualtitative_results}. Since our train and test data come from the same video sequences, we assume that they are correlated, which would affect our results. In order to evaluate the capabilities of our model to generalize to completely unknown data, we use a setup with two short video sequences without any overlap or known objects displayed, but similar conditions like camera angle or weather. We train on the first and then evaluate on the second sequence. The results are in average $30$\,\%\xspace worse than with combined training. We conclude that the model generalizes rather moderately to unknown data. However, this could most likely be improved by a larger and more diverse database, as the experimental set-up presented here corresponds to an extreme case. Normally the base model should contain at least some scenes that are similar to the test scene.

%\subsection{Unstable training on low batch sizes}
%\label{sec:unstable_training}
%We observe very unstable training on low batch sizes. Particularly in early iterations the model tends to diverge and get stuck in this local minimum. To effectively prevent this, we use a batch size of $20$ or higher. We assume this problem arises from our pose estimation, because especially datasets with complex camera movement, in particular high amounts of rotation without forward motion are affected. One possible explanation for this issue might be our shared encoder architecture. Since our pose estimation is depth-based and our depth estimation needs pose information to learn, this could potentially create a vicious circle for datasets with difficult camera movements. High batch sizes might minimize the probability of multiple problematic camera movements processed in one batch and prevent divergence in early training iterations. After the network starts to predict reasonable death maps the batch size can be dropped. In our experiments batch sizes above $20$ do not tend to produce better results. 

%\subsection{Continual Learning}
%\label{sec:continual_learning}
%The rather poor generalization in this state with this database prevents a application on completely unknown data. Since our method is self-supervised and does not require ground truth depth data, the distinction between training phase and practical application is not as sharp as in classical supervised learning. We developed an approach to fine tune our model on unknown data to further improve the performance. To measure the advantages of such a method we use two sequences of images. Sequence \textit{A} is used to train a base model until convergence. Then we continue training with the second sequence \textit{B} and measure the improvements constantly. As shown in figure \ref{fig:relearn_switch} the performance of sequence \textit{B} rapidly improves while the results on sequence \textit{A} degrade. This fine tuning is about $10$ times faster then normal training with equal results. To prevent unlearning sequence \textit{A} we use combined fine tuning with both sequences which gives similar results, but is slower because the dataset is bigger. The progress of this training is shown in figure \ref{fig:relearn_continue}. Depending on the intended use, the first or second approach is relevant, depending on whether it is important to keep the known scenes and how crucial the speed is. In both cases, a base model that is as diverse as possible should be advantageous and can then be adapted for specialized use cases. But the method of continual learning also has disadvantages, because in contrast to the normal application the pose estimation is now also needed. In addition, not only the forward pass through the network must be calculated, but also the weight adjustment in the backward pass. 
%
%\begin{figure*}
%    \centering
%    \begin{minipage}{.5\textwidth}
%      \centering
%      \includegraphics[width=8cm]{figures/relearn_switch_a1_ni.pdf} 
%      \caption{Switching from sequence \textit{A} to \textit{B}}
%      \label{fig:relearn_switch}%  
%    \end{minipage}%
%    \begin{minipage}{.5\textwidth}
%      \centering
%      \includegraphics[width=8cm]{figures/relearn_continue_a1_ni.pdf}    
%    \caption{Fine tuning on both sequence \textit{A} and \textit{B}}%
%    \label{fig:relearn_continue}%
%    \end{minipage}
%\end{figure*}

==> chapters/07_acknowledgments.tex <==
\section*{ACKNOWLEDGEMENTS}
\label{sec:acknowledgments}
